SocialFilter: Collaborative Spam Mitigation using Social Networks

Spam mitigation can be broadly classified into two main approaches: a) centralized security infrastructures that rely on a limited number of trusted monitors to detect and report malicious traffic; and b) highly distributed systems that leverage the experiences of multiple nodes within distinct trust domains. The first approach offers limited threat coverage and slow response times, and it is often proprietary. The second approach is not widely adopted, partly due to the lack of guarantees regarding the trustworthiness of nodes that comprise the system. Our proposal, SocialFilter, aims to achieve the trustworthiness of centralized security services and the wide coverage, responsiveness and inexpensiveness of large-scale collaborative spam mitigation. We propose a large-scale distributed system that enables clients with no email classification functionality to query the network on the behavior of a host. A SocialFilter node builds trust for its peers by auditing their behavioral reports and by leveraging the social network of SocialFilter administrators. The node combines the confidence its peers have in their own reports and the trust it places on its peers to derive the likelihood that a host is spamming. The simulation-based evaluation of our approach indicates its potential under a real-world deployment: during a simulated spam campaign, SocialFilternodes characterized 92% of spam bot connections with confidence greater than 50%, while yielding no false positives

==> implementation.tex <==
\section{Implementation}

In this section, we describe FaceTrust's software components.
We have currently implemented portions of this software
architecture, and we defer complete implementation and 
deployment to future work. 
We provide a description of the RPC API that FaceTrust node offers 
to other applications as well as the RPC APIs that the distributed
repository and the OSN provider offers to FaceTrust nodes.
We provide this description to offer further insights
on the design and operation of our system.

\subsection{FaceTrust Software Architecture}
\label{subsec:facetrust-software-architecture}

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.3]{figures/FaceTrust-Software-Architecture.eps}
\caption{\label{fig:facetrust-architecture} FaceTrust software architecture.}
%A figure describing the Facebook application, the FaceTrust
%demon/client and the messages they exchange. They both run on the same machine.
%In addition, there is the Facebook application server.
\end{center}
\end{figure}

We now describe how users are expected to deploy and use FaceTrust.
Every user that wishes to join the FaceTrust network and enable
his applications to retrieve and report trust on their observed
Internet traffic takes the following steps: a) installs an OSN application,
e.g. a FaceTrust Facebook application; b) installs a FaceTrust demon
application, which communicates with the Facebook application and joins
the FaceTrust overlay.

Figure~\ref{fig:facetrust-software-architecture} describes our systems
software architecture. The first component the system comprises of 
is the FaceTrust demon application,
which runs the FaceTrust logic described in Section~\ref{subsec:design}.
It is responsible for: a) joining the distributed DHT repository, storing
and resolving queries for behavioral reports and trust updates; b) connecting
to FaceTrust nodes in its view and retrieving their public keys; c) obtaining
behavioral reports and direct trust updates between nodes in its view; d) aggregating
trust values and deriving a trust value with respect to entities and their actions.

The second component is the OSN application, e.g. a Facebook application. This
is a widget that runs from within the OSN providers website and enables a user
to: a) register with the FaceTrust network and retrieve a public/private key pair
which it uses to configure its FaceTrust client(demon); b) look for other FaceTrust users
in his social network; c) assign social trust values to users in its network that
also use FaceTrust; d) communicate the social trust values between the user and its friends
admins to the FaceTrust demon to enable it to initialize its trust graph. Typically
the FB app submit the social trust to the application server, and the FT demon
retrieves it from it using the FB API.

The third component is the FaceTrust Facebook aplication server. The server 
is tasked with: a) issuing public key certificates; b) assigning identity
trust values for each node by analyzing the social graph; c) registering the social trust values between
nodes and sending them to nodes upon request; d) tracking facetrust nodes and
returning a random view of online FaceTrust nodes (IP, port) to new nodes
that wish to join the network. Each node gets a restricted view of the network from 
the tracker to mitigate manipulation by malicious nodes; 
%the tracker keeps track of what view it returns to each node
d) providing FaceTrust nodes with the contact
information of a randomly chosen node, which they use to join the Chord DHT.



\subsection{Distributed Repository}

In our simulations, we use the Chord~\cite{Stoica-SIGCOMM-01} 
Distributed Hash Table. Our implementation uses  a 160-bit circular id space. 
In our simulations, we use the Chord~\cite{Stoica-SIGCOMM-01} Distributed Hash Table.
Chord uses a 160-bit circular id space. Unlike Pastry,
Chord forwards messages only in clockwise direction in
the circular id space. Instead of the prefix-based routing
table in Pastry, Chord nodes maintain a routing table consisting
of up to 160 pointers to other live nodes (called a
“finger table”). The ith entry in the finger table of node n
refers to the live node with the smallest nodeId clockwise
from $n+2^{i-1}$. The first entry points to n’s successor, and
subsequent entries refer to nodes at repeatedly doubling
distances from n. Each node in Chord also maintains
pointers to its predecessor and to its n successors in the
nodeId space. This successor list represents a node's neighbor
set. Chord’s replica function maps an object’s key to the nodeIds in 
the neighbor set of the key’s root, i.e., replicas are stored in the neighbor
set of the key’s root for fault tolerance. The expected
number of routing hops in Chord is $\frac{1}{2}\log_2 N.$

Table~\ref{fig:facetrust-repository-api} presents the API that
the distributed FaceTrust repository exports to FaceTrust nodes.

FaceTrust nodes may obtain their view of the FaceTrust overlay $V$
using the {\tt node\_list get\_view()} function. FaceTrust nodes submit behavioral
reports for entities they encounter using the {\tt submit\_behavioral\_report()} function. Nodes
receive behavioral reports that are submitted by nodes in their view using
the {\tt get\_behavioral\_report()} function. The {\tt action} 
argument takes values that specify the malicious action with which the entity is associated, 
such as  ``host is spam bot'', ``packet carries worm'', ``email signature is spam'', 
``host is DDoS attacker'', ``host is malware server'' etc.
The {\tt entityID} argument describes the identity of the entity for which
the report is submitted. For example, a report with action ``packet carries worm''
uses as ID the hash of the packet. The {\tt trust} argument specifies how confident 
the sender node is that this report is correct. The {\tt nodeID} argument
specifies which node's behavioral report to retrieve.

FaceTrust nodes also  retrieve direct trust updates $d_{ij}$ for nodes in their 
view, when both $i,j\in V$, by using the {\tt get\_direct\_trust()} function. 
The {\tt nodeID} argument corresponds to the node this trust update concerns.
Nodes submit  reporter trust updates using the 
{\tt submit\_direct\_trust()} function.


\begin{table*}[t!]
\begin{center}
\begin{tabular}{p{3.1in}|p{3.1in}}
\multicolumn{2}{c}{{\it FaceTrust Repository RPC API}} \\
\hline
{\bf Name} & {\bf Purpose} \\
\hline
\hline
{\tt void submit\_behavioral\_report(action,entityID,trust))}  & 
Submit a behavioral report to the repository of the type {\tt action}
concerning the entity {\tt entityID} with confidence {\tt trust}. \\
{\tt  trust get\_behavioral\_report(entityID, action, node\_list))}  & 
Retrieve a behavioral report from the repository of the type {\tt action}
concerning the entity {\tt entityID} that has been submitted by nodes in {\tt node\_list}. \\
\hline
{\tt trust get\_reporter\_trust(
void (*reporter\_trust\_update)(admin* sender, admin* reporter, trust*))}  &
Registers a callback to be called 
when the repository receives a reporter trust update from the {\em sender} admin
in $V$ regarding the {\em reporter} admin in $V$. \\
\hline
{\tt void* send\_behavioral\_report(type\_of\_report*, description*, trust*)} &
Called to submit behavioral reports to the repository. \\ 
\hline
{\tt void* send\_reporter\_trust\_update(adminID* reporter, reporter\_trust*)} &
Called to submit trust updates concerning a reporter admin.
to the repository. \\ 
\hline
\end{tabular}
\end{center}
\caption{API for the FaceTrust Repository, for
receiving and sending behavioral reports and reporter trust updates.}
\label{fig:facetrust-repository-api}
\end{table*}
% end table


\subsection{Online Social Network Provider API}

Table~\ref{fig:facetrust-osn-api} presents the API that
a FaceTrust-enabled online Social Network Provider exports to FaceTrust nodes.
The OSN provider is responsible for running the Facebook Application server
discussed in Section~\ref{subsec:facetrust-software-architecture}.

\begin{table*}[t!]
\begin{center}
\begin{tabular}{p{3.1in}|p{3.1in}}
\multicolumn{2}{c}{{\it FaceTrust Social Network API}} \\
\hline
{\bf Name} & {\bf Purpose} \\
\hline
{\tt public\_key* get\_public\_key(admin*)} & 
Returns the cryptographic public key of the specified {\em admin}.\\
\hline
{\tt trust* get\_identity\_trust(admin*)}  & 
Returns a value in $[0.0,1.0]$ that indicates the trust that the OSN
provider has the specified {\em admin} is not performing a Sybil attack. \\
\hline
{\tt trust* set\_social\_trust(admin*)} &
Sends to the OSN provider a value in $[0.0,1.0]$ that reflects the amount of trust 
the callee places to the specified {\em admin} through means
of direct personal acquaintance. It is used by FaceTrust nodes to store
with the OSN provider how much social trust they place on their acquainted admins.\\
{\tt trust* get\_social\_trust(admin*)} &
Returns a value in $[0.0,1.0]$ that reflects the amount of trust 
the callee places to the specified {\em admin} through means
of direct personal acquaintance. It is used by the FaceTrust
nodes to retrieve the social trust in case they reset. \\
{\tt node\_list get\_view()} & 
Retrieves a partial view of nodes in the FaceTrust overlay.\\
\hline
\hline
\end{tabular}
\end{center}
\caption{C-style API for the FaceTrust Online Social Network Application
server, for the issuance of a public key certificate, for determining a node's
identity trust and for retrieving a partial view of the FaceTrust network.}
\label{fig:facetrust-osn-api}
\end{table*}
% end table


\subsection{FaceBook Application}

% this content is from http://developers.facebook.com/documentation.php
The FB Platform is a standards-based web service with methods for accessing and
contributing FB data \cite{facebook-platform}. It comprises the following parts:
(i) the FB API, which %uses a REST-based interface.
\if 0
FB method calls are made over the internet by sending HTTP GET
or POST requests to a REST server.
\fi
%The API
enables developers to add social context to their application by
utilizing data regarding the user's profile, its friends, its pictures, and events;
(ii) the FB Query Language (FQL), which resembles an SQL interface to
access the same data that one can access through the FB API;
iii) Markup (FBML) and Java Script (FBJS), which allow developers to build applications 
that integrate into a user's FB experience through the Profile, Profile Actions, Canvas, 
News Feed and Mini-Feed.

Fig. 1 shows aspects of the Facebook Developer Platform’s
architecture that are relevant to our applications. In
this architecture, a user interacts indirectly with the application
servers through Facebook’s API servers. This enables
Facebook to protect users from malicious content that may
be embedded in the response data by the application servers,
since Facebook can process and strip undesirable content

We must note, however, that Facebook has an alternate
method for deploying applications on its Platform that enables
users to interact directly with the application servers

However, the architecture shown in Fig. 1 is the dominant
architecture used, primarily due to the ease of displaying
content to the application users3 and the protection of the
application servers’ identity from the end-users. We adopt
this architecture to develop our own Facebook applications
to limit the resources required to render content to users.
This architecture relieves application servers from the the
extra task of downloading and uploading extra content, such
as users’ real names and graphical content from Facebook.

\subsection{FaceTrust Client API}

We now provide a detailed description of the API that FaceTrust nodes
offer to applications tasked with detecting or possibly handling unwanted traffic.
A {\em FaceTrust node} uses the {\tt Report(entityID, action, confidence)}
interface to feedback its observed behavior of an entity to the repository. 
Each report includes a timestamp and is signed by the reporting
FaceTrust node's public key for authentication and
integrity. FaceTrust nodes compute the trust metric {\tt
GetTrust(entityID, action)} by aggregating relevant reports in the
repository. An end system that does not participate in FaceTrust
may be configured to send {\tt GetTrust} calls to FaceTrust nodes 
it trusts, or that reside in their local administrative domains, 
similar to the DNS system.

\begin{table*}[t!]
\begin{center}
\begin{tabular}{p{3.1in}|p{3.1in}}
\multicolumn{2}{c}{{\it FaceTrust API}} \\
\hline
{\bf Name} & {\bf Purpose} \\
\hline
{\tt public\_key* get\_public\_key(admin*)} & 
Returns the cryptographic public key of the specified {\em admin}.\\
\hline
{\tt trust* get\_identity\_trust(admin*)}  & 
Returns a value in $[0.0,1.0]$ that indicates the trust that the OSN
provider has the specified {\em admin} is not performing a Sybil attack. \\
\hline
{\tt trust* get\_social\_trust(admin*)} &
Returns a value in $[0.0,1.0]$ that reflects the amount of trust 
the callee places to the specified {\em admin} as inferred
by the social graph. \\
\hline
\hline
\end{tabular}
\end{center}
\caption{C-style API for the FaceTrust API that FaceTrust nodes
offer to applications.}
\label{fig:facetrust-osn-api}
\end{table*}



\subsection{PGP wef of Trust with ID trust}
3) Implementation: FaceTrust identity trust plugin for BGP key distribution.

